Learning Generalizable Robotic Reward Functions from "In-The-Wild" Human Videos

We are motivated by the goal of generalist robots that can complete a wide range of tasks across many environments. Critical to this is the robot's ability to acquire some metric of task success or reward, which is necessary for reinforcement learning, planning, or knowing when to ask for help. For a general-purpose robot operating in the real world, this reward function must also be able to generalize broadly across environments, tasks, and objects, while depending only on on-board sensor observations (e.g. RGB images). While deep learning on large and diverse datasets has shown promise as a path towards such generalization in computer vision and natural language, collecting high quality datasets of robotic interaction at scale remains an open challenge. In contrast, "in-the-wild" videos of humans (e.g. YouTube) contain an extensive collection of people doing interesting tasks across a diverse range of settings. In this work, we propose a simple approach, Domain-agnostic Video Discriminator (DVD), that learns multitask reward functions by training a discriminator to classify whether two videos are performing the same task, and can generalize by virtue of learning from a small amount of robot data with a broad dataset of human videos. We find that by leveraging diverse human datasets, this reward function (a) can generalize zero shot to unseen environments, (b) generalize zero shot to unseen tasks, and (c) can be combined with visual model predictive control to solve robotic manipulation tasks on a real WidowX200 robot in an unseen environment from a single human demo.

==> algoblock.tex <==
\begin{algorithm}[H]
\caption{\textsc{\algo}: Training phase}
\begin{algorithmic}[1]
\STATE \textbf{Require:} $\{\D_{i}^h\}$ human demonstration data for a set of tasks $\{\T_i\} \sim p(\T)$
\STATE \textbf{Require:} $\{\D_{j}^r\}$ robot demonstration data for a set of tasks $\{\T_j\} \subseteq \{\T_i\}$
\STATE \textbf{Require:} Pre-trained video encoder $f_{enc}$
\STATE Randomly initialize similarity discriminator $f_{sim}$
\WHILE{training}
\STATE Sample video $d_k \in \D^h \cup \D^r$
\STATE Sample videos $d_k^*, d_l \in \D^h \cup \D^r \setminus {d_k}$
\STATE $h_k, h_k^*, h_l \leftarrow f_{enc}(d_k), f_{enc}(d_k^*), f_{enc}(d_l)$
\STATE $\L = \L_{CE}(f_{sim}, h_k, h_k^*) + \L_{CE}(f_{sim}, h_k, h_l)$
\STATE Update $f_{sim} \leftarrow f_{sim} - \alpha \nabla_{f_{sim}} \L$
\ENDWHILE{\textbf{end while}}
\end{algorithmic}
\end{algorithm}

\vspace{-0.3cm}
\vspace{-0.3cm}

\begin{algorithm}[H]
\caption{\textsc{\algo}: Planning from videos}
\begin{algorithmic}[1]
\STATE \textbf{Require:} Pre-trained video encoder $f_{enc}$
\STATE \textbf{Require:} Pre-trained video prediction model $f_{pred}$
\STATE \textbf{Require:} Trained similarity discriminator $f_{sim}$
\STATE \textbf{Require:} $K$ videos $\{d^{(i)}\}$ for task $\T$
\STATE Encode $\{h^{(i)}\} \leftarrow \{f_{enc}(d^{(i)})\}$
\FOR{trials $1, ..., n$}
    \FOR{$t$ trajectories}
    \STATE Run MPC/CEM with $f_{pred}$:
    \STATE Sample actions $\{a_{1:l}\}$ and get predicted trajectories $\{\tilde{s}_{1:l}\} \leftarrow \{f_{pred}(s_0, a_{1:l})\}$
    \STATE Encode $\{h_{1:l}\} \leftarrow \{f_{enc}(\tilde{s}_{1:l})\}$
    \FOR{each $h_{1:l}$}
    \STATE Calculate similarity score $S_{h_{1:l}} = \frac{1}{K}\sum_{i} f_{sim}(h_{1:l}, h^{(i)})$
    \ENDFOR{}
    Take $a_{1:l}$ with the largest corresponding $S_{h_{1:l}}$
    \ENDFOR{}
\ENDFOR{}
\end{algorithmic}
\end{algorithm}

